Physion: Evaluating Physical Prediction from Vision in Humans and Machines

While current vision algorithms excel at many challenging tasks, it is unclear how well they understand the physical dynamics of real-world environments. Here we introduce Physion, a dataset and benchmark for rigorously evaluating the ability to predict how physical scenarios will evolve over time. Our dataset features realistic simulations of a wide range of physical phenomena, including rigid and soft-body collisions, stable multi-object configurations, rolling, sliding, and projectile motion, thus providing a more comprehensive challenge than previous benchmarks. We used Physion to benchmark a suite of models varying in their architecture, learning objective, input-output structure, and training data. In parallel, we obtained precise measurements of human prediction behavior on the same set of scenarios, allowing us to directly evaluate how well any model could approximate human behavior. We found that vision algorithms that learn object-centric representations generally outperform those that do not, yet still fall far short of human performance. On the other hand, graph neural networks with direct access to physical state information both perform substantially better and make predictions that are more similar to those made by humans. These results suggest that extracting physical representations of scenes is the main bottleneck to achieving human-level and human-like physical understanding in vision algorithms. We have publicly released all data and code to facilitate the use of Physion to benchmark additional models in a fully reproducible manner, enabling systematic evaluation of progress towards vision algorithms that understand physical environments as robustly as people do.

==> Revisions/representation_learning.tex <==
% (5) Distinction between model training and readout fitting. In general, we will revise and expand section 2.4 to make the process of model training and readout fitting clearer and to better explain why we divide model evaluation into these two steps. In the original manuscript, “y” denotes the binary ground truth class label (contact or no contact), which P(contact) (i.e. the predicted class label \hat{y}) should be optimized to match. We will make the terminology consistent. 

% Model training and readout fitting are distinct, and thus require distinct datasets (see response to point (3) above.) In this work, training sets were used to optimize parameters of visual encoders and/or forward dynamics models -- i.e., models that predict what is going to happen next from an initial sequence of frames. Our model training protocols included mixing all the scenarios’ training sets together, for a total of 16,000 movies each 5 seconds or longer. Importantly, though, *we did not optimize models to do the OCP task directly* during the training stage. While this is theoretically possible to do using the OCP class labels in the training datasets, it would not help us assess whether any models have or can acquire human-like representations of the physical world (see below.) Rather, we use the *readout fitting sets* to train models to do the OCP task. Specifically, we use these datasets to fit general linear models (e.g. logistic regressions) from the pretrained encoder and dynamics model features to the OCP class labels y *for a single one of the eight scenarios.* Readout fitting is really meant to play the same role as the Familiarization trials play in human experiments: a way of indicating how people or models can apply their existing representations and knowledge to do a particular psychophysics task, which may not be like any task they have previously encountered. Ideally, model readout fitting would be done only with the same 10 trials people saw during Familiarization, but here we provide two orders of magnitude more trials to make up for the fact that people in our task can follow language-level instructions, whereas the models tested here cannot.

% We will clarify in our revised manuscript why we do not train models directly on the OCP class labels of the training sets. In essence, it is because we are interested in *unsupervised representation learning* about the physical world, akin to unsupervised pretraining of vision or language models; we want to assess how well models trained by some other objective -- and possibly on some other dataset with more scenes and greater realism -- can *transfer* to making OCP predictions in the Physion task. This is different from supervising all of a large model’s parameters to predict the OCP class label directly on the Physion training data, which might yield models that “solve” the task (especially since the training data were drawn from the exact same distributions as the testing data) but almost certainly would yield weak, non-general representations. This would be analogous to training a large vision model with supervision to read a set of barcodes: the model might well succeed (and exceed human performance) but there is no reason to expect that it would transfer well to other visual tasks. We plan to make this logic explicit in our revision and acknowledge that it is somewhat different from other benchmarks for physical prediction, where models have usually only been tested for their ability to do a single task on a single scenario with significant supervision.

% Another way to think about this choice is that many of the models we test from the literature have a specifically-chosen loss function that is *part* of the model specification -- it’s not just the “architecture”  of the network that counts, but also the signal on which its representation is trained. If we had instead ripped off the original training heads of the models, and then trained just the architectures end-to-end to solve our specific red-object-hit-yellow-zone problem, that would have *not* provided a real test of what the original model creators intended. Or rather, it would just be a test of their “architecture” but not the learning signals -- and we, intentionally, explicitly seek to test the “whole models”, with their constitutive learning signals, in our benchmark.

%% paragraph for the intro?
% We intend the \textbf{Physion} benchmark to be a tool for measuring how well an algorithm perceives the physical structure and dynamics of commonplace phenomena, akin to how computer vision datasets like ImageNet \citep{deng2009imagenet} and SVHN XXX are used to assess learned representations for object recognition.
% We expect that an algorithm that truly ``understood'' everyday physics the way humans do would not need extensive training on data from \textbf{Physion} or supervision on the OCP task, since people only needed 10 familiarization trials with feedback to perform accurately.
% Thus, although we provide large training datasets for each of the \textbf{Physion} scenarios, we intend for these data to be used mainly for \textit{unsupervised} fine-tuning or for training from scratch on inputs that are not widely available in other large computer vision datasets (such as particles generated from each ground truth object mesh.)
% These training data are generated from the same distribution of physical configurations as the \textbf{Physion} testing sets.
% For this reason, obtaining high testing set accuracy on one or more scenarios \textit{via} supervision would not indicate that a machine learning model had acquired human-like physical representations, any more than overfitting a high-capacity model to a narrow supervised task (like distinguishing two object categories) would indicate human-like visual ability.
% We want to test hypotheses, instantiated as computational models, about how human adults acquire a rich understanding of the physical world and an ability to predict how scenes will unfold; 
% since machine learning models are defined by both their architecture and the learning signals used to train them, we think these hypotheses are best tested if OCP labels are not provided during training.
% Ideally, then, \textbf{Physion} will serve as a challenging test of \textit{unsupervised representation learning about the physical structure of visual scenes.}

%%% JEFAN notes 11/1/21: I like a lot of the content in these paragraphs, and I am thinking about the best way to integrate it into the Introduction. Rather than tacking it on at the end, it seems like it'd be helpful to describe the intended use cases as close to where we describe our key contributions as we can. 
%%% In that same spirit, I think it may be helpful to have a bit more structure in the Intro, overall -- perhaps with subsection headers and very explicit declarations of what we take our contributions to be. 
%%% Perhaps following the outline from the talk? Like (1) fact that Physion comes with not only the dataset, but a dataset *generation procedure* can be grouped together as one point. Then (2) the task/evaluation protocol is envisioned as being useful for evaluating any model pre-trained under whatever objective. (3) Then the results could all be integrated together, to reduce overlap between what's currently in this paragraph and what's currently the final paragraph in the intro. 
%% add to the intro
\textbf{Our Vision for Physion.}
Our public release of \textbf{Physion} includes large, labeled training sets for each scenario as well as code for generating unlimited additional training data -- or even designing new scenarios with new types of visual diversity and physical phenomena.
As such, \textbf{Physion} may be used -- as machine-learning datasets and benchmarks often are -- for training models directly on the benchmark task for one or more of the scenarios, yielding (for instance) a model that excels at predicting whether the towers in the \textbf{Support} scenario will fall.
However, our main intent is for \textbf{Physion} to \textit{test how well pretrained models transfer to challenging physical understanding tasks} -- in other words, to compare model to human ability as directly as possible.
People are able to make accurate predictions about \textit{Physion} videos without prior experience of our simulation environment or explicit supervision on the Object Contact Prediction task.
Thus, \textbf{Physion} provides a way to compare models' to humans' \textit{task-general} representations of the physical world and its dynamics, with Object Contact Prediction meant as a way to interrogate these representations rather than as a task to be optimized for directly.
In identifying particular scenarios or conditions where models' physical knowledge fall short of a person's, \textbf{Physion} should further help to diagnose which model components are lacking.
We demonstrate this usage by comparing a range of computer vision models that fare poorly on \textbf{Physion} to ``positive control'' models that succeed: ones that receive a physical explicit scene representation, rather than videos, as their input.
These results suggest that a major missing ingredient in computer vision models is explicit representation of objects and their physical properties, which may be prerequisite for predicting how scenes will unfold over time.

%% Add to methods about "batches" of stimuli drawn from parameters

%% Add to methods ~L118
\textbf{Representation Learning \textit{versus} Readout Fitting}
\textbf{Physion} is meant for testing a wide range of computer vision models, which vary greatly in their architecture and optimization procedures.
We do not want to restrict testing to models trained on a narrow task like Object Contact Prediction or even to models trained on prediction-related loss functions: 
it is possible that a model trained on an ``unrelated'' task like object recognition has acquired a partly human-like representation of the physical world, which benchmarking on \textbf{Physion} should be able to reveal.
For this reason, we divide the model evaluation procedure into two stages: \textit{representation learning} and \textit{readout fitting}.
Representation learning may include pretraining of a model architecture on any task and dataset prior to transfer to the \textbf{Physion} data.
For models that do not explicitly predict the temporal dynamics of a scene representation, this stage also includes training of a forward dynamics model on the \textbf{Physion} scenarios.
Importantly, dynamics training is \textit{unsupervised} with respect to the Object Contact Prediction task: models do not receive task labels, are not cued to particular objects, and may train on video clips from all parts of \textbf{Physion} trials, not just the beginning.
The purpose of this training is for models to learn or fine-tune their representations of physical dynamics using their original architectures and loss functions.

In contrast, readout fitting is meant to adapt a pretrained model to the Object Contact Prediction task without changing its underlying representation of physics. 
The reason an adaptor is needed is that for most neural network models, an answer to the question "Did the red object hit the yellow object?" cannot be inferred directly from model activations; most neural networks do not even explicitly represent distinct objects.
In readout fitting we therefore freeze the parameters of a pretrained neural network and fit a generalized linear model on different subsets of model features (see below), with the ground truth object contact labels acting as supervision.
Moreover, in order to train a linear readout that will be effective on the testing stimuli, the readout fitting stimuli must be drawn from the same distribution as the testing stimuli in terms of both visual statistics and physical dynamics.
We therefore provide two distinct sets of training stimuli for each scenario in \textbf{Physion}: a \textit{dynamics training set} of trials created from the same underlying physical parameters as the testing stimuli, but without visual cues that indicate an agent and a patient object; and a \textit{readout fitting set} with both physical dynamics and visual cues (i.e., red agent and yellow patient objects) matched to the testing set.
For readout fitting and testing, only the first 1.5 seconds of each trial is shown to the pretrained model.






==> Sections/checklist.tex <==
\section{Paper Checklist}

\begin{enumerate}
    \item For all authors...
    \begin{enumerate}
        \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? \textbf{Yes.}
        \item Have you read the ethics review guidelines and ensured that your paper conforms to them? \textbf{Yes.}
        \item Did you discuss any potential negative societal impacts of your work? \textbf{Yes.}
        \item Did you describe the limitations of your work? \textbf{Yes.}
    \end{enumerate}
    \item If you ran experiments...
    \begin{enumerate}
        \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? \textbf{Yes, see \url{https://github.com/cogtoolslab/physics-benchmarking-neurips2021}.}
        \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? \textbf{Yes, see training protocol in Supplement and \url{https://github.com/neuroailab/physopt-physics-benchmarking}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)? \textbf{Yes.}
        \item Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? \textbf{Yes, see \ref{A2:computational_details}.}
    \end{enumerate}
    \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
    \begin{enumerate}
        \item If your work uses existing assets, did you cite the creators? \textbf{Yes, see \ref{A2:computational_details}.}
        \item Did you mention the license of the assets? \textbf{Yes, see \ref{license}}
        \item Did you include any new assets either in the supplemental material or as a URL? \textbf{Yes, we have provided a URL to our GitHub repository which includes scripts to automatically download all new assets associated with our paper.}
        \item Did you discuss whether and how consent was obtained from people whose data you're using/curating? \textbf{Yes, consent was obtained via an online form that was presented to each participant before they began the study. Only participants who provided consent were included in our dataset and analyses.}
        \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content? \textbf{We did not collect any personally identifiable information from participants in our studies, in accordance with our IRB protocol. We further anonymmized any participant identifiers prior to making the behavioral datasets publicly available. None of our data contain any offensive content.}
    \end{enumerate}
    \item If you used crowdsourcing or conducted research with human subjects...
    \begin{enumerate}
        \item Did you include the full text of instructions given to participants and screenshots, if applicable? \textbf{Yes, we have included these details in our figures and description of the task procedure. In addition, we have also made the code that was used to run our human studies publicly available for review.}
        \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable? \textbf{Yes. All human behavioral experiments were conducted in accordance with the UC San Diego IRB.}
        \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation? \textbf{Yes. We provided \$12/hour compensation to the human participants in our studies. We determined this hourly wage based on the minimum wage in California in 2020. We expect to increase this wage on pace with changes in state and federal policy. }
    \end{enumerate}
\end{enumerate}

==> Sections/conclusion.tex <==
\section{Discussion}

==> Sections/design.tex <==
\section{Benchmark Design \textcolor{MyPurple}{Dan B}}
% Benchmark Design

\begin{figure}[t]
\centering
    \includegraphics[width=0.3\textwidth]{Figures/figure1 - task schematic.png}
\vspace{-7.5pt}
\caption{Cartoon schematic of the OCP task}
\label{fig:ocp_schema}
\vspace{-15pt}
\end{figure}

% P4: Types of scenarios / physics tested here

% SS1: General considerations for our benchmark
\subsection{General Considerations for Testing Intuitive Physics}

% P1: Problems with collecting many aspects of intuitive physics into a single dataset/benchmark: What unifies them? How to get around language-level tasks for abilities that we think are pre-/non-linguistic?
Many high-quality benchmarks have helped push the development of visual algorithms for \textit{semantic} scene understanding -- how a person might describe the types of object present, the actions occurring, and the high-level content or relationships between things.
We mean to test an orthogonal set of human visual abilities -- ``visual intuitive physics'' (VIP) -- that do not require categorical classification or semantic understanding: those that allow us to perceive novel objects and predict how they will physically behave and interact with other objects, even without knowing what categories they belong to.
Although videos from existing vision datasets and benchmarks \textit{involve} physical phenomena, their use of everyday objects and scenes confounds tests of physical understanding with tests of semantic knowledge.
A model for predicting where cups stand in relation to plates and tables might learn only spatial correlations between these object categories, without ever learning what would happen if a cup were placed on its side or on the edge of a table.
This implies that a VIP benchmark task should not be solvable through semantic understanding of scenes or knowledge of which object configurations are common in the real world; 
rather, it should require judgments about objects' physical properties, relationships, and dynamics.

% P2: OCP task design as a way to get around language-induced classification and focus on the physics; one extreme is trajectory prediction
This poses a new question, though: \textit{which} properties, relationships, and dynamics? 
At one extreme, a VIP task could ask participants to predict the precise spatiotemporal trajectories of multiple objects, as in some existing benchmarks that test on billiards or billiards-like scenarios.
However, the ability to make such predictions is not common in humans outside of highly constrained scenarios -- even judging how a billiards shot will unfold is an expert-level skill -- and, we argue, is not the essence of visual intuitive physics.
In trying to grasp a coffee mug, deciding whether a cup is safely supported by a saucer, or noticing that a piece of debris might roll in front of the car, a person will \textit{ignore} or \textit{approximate} most low-level physical scene variables even if they could estimate them accurately in principle: intuitive physical understanding involves knowing which aspects of a scene are most relevant to possible and likely outcomes of interest.

% P2b: opposite extreme is asking simple questions
This observation has motivated physical understanding tasks that lie at the opposite extreme of precise trajectory prediction: answering basic questions about what will or might happen as a scene unfolds.
For instance, XXX and XXX ask participants whether a stack of toy blocks will fall over or two objects will collide and design models that also output answers to these yes-or-no questions.
In these cases, the tasks are designed under the assumption that certain physical, higher-order variables -- the persistence of the block tower and the presence of a collision at \textit{any} time in the near future -- are more important than the lower-level physical interactions and processes that give rise to them.
This is far closer than trajectory prediction to what we think of as intuitive physical understanding.
The main downside of this task design is that there are many aspects of VIP that are expressed awkwardly in natural language: 
testing whether an algorithm could understand the elaborate mechanism of a ``Rube Goldberg device'' might require dozens of questions, whereas a person could ``just see'' how it was likely to work.

% P2c: OCP is a good intermediate
We have therefore created a happy medium between these two extremes: \textit{object contact prediction} (OCP), a task that combines the greater higher-order understanding requirement of question answering with the more ``intuitive,'' less language-dependent nature of full trajectory prediction.
In OCP, a person or model is shown the first $T_{\texttt{vis}}$ frames of a $T > T_{\texttt{vis}}$ movie that depicts some physical scenario, such as a ball about to collide with a tower of blocks. 
They are then asked to predict whether two of the objects in the scene -- termed the \textit{agent} and the \textit{patient} object -- will come into contact at any time before all the objects in the scene have come to complete rest (frame $T$).
In the simplest version of this task, the agent and patient objects are indicated by pre-task instructions as having certain visual features that uniquely specify them in every trial, e.g. the task is always to predict whether the sole red object and the sole yellow object will touch.
In a version more in line with standard visual psychophysics tasks, the two objects are \textit{pre-cued} for each trial by overlaying transparent segmentation masks on the agent and patient objects.
The pre-cuing version is more flexible, as it allows the same movie to be used as different task trials by changing only which objects are indicated as agent and patient;
whereas the uniform feature-based cueing version is better suited for testing computer vision models, since it requires only standard visual input and a visual representation that is sensitive to the cued features.
Importantly, people make essentially the same predictions on both task versions, so human-like performance on either one by a computer vision model would be consistent with human-like physical understanding.

% P3: How the OCP task + a simulator addresses the desiderata
The OCP task design allows us to probe many aspects of VIP, some of which are not easily put into words, by programmatically placing objects and setting them in motion.
In judiciously arranged scenes, contact between agent and patient objects merely serves as a non-verbal indicator of some physical higher-order variable -- whether a tower fell over, a bowl contained a ball, a torus was attached to a post, and so on (Fig XXX).
Thus, a person or model could be expected to solve this task if and only if it understood higher-level properties of the underlying physics, but would not need to learn a mapping from language-level categories to visual input or physical predictions.
It is easier to create a large and diverse set of such scenarios (which is necessary for training machine learning algorithms) with a highly visually and physically realistic simulator than with real objects.
We therefore use ThreeDWorld, a Unity3D-based environment XXX
TDW also provides multiple modalities of visual data and the full ground truth state of objects in the physical simulation, which makes it possible to test which types of visual and physical information are most important for an algorithm to ``see'' during training and evaluation to make physical predictions.
For this first public version of our benchmark, we have developed eight scenarios that each incorporate different aspects of intuitive physics (Table XXX and Figure XXX.)
Additional scenarios will be developed that incorporate other physical phenomena common to everyday life (e.g. ``squishy'' materials and fluid dynamics), and custom scenarios can be straightforwardly designed by modifying or combining existing ones using our public code XXX.

\begin{figure}[t]
\centering
    \includegraphics[width=0.98\textwidth]{Figures/scenario_display_v0.pdf}
\vspace{-7.5pt}
\caption{PLACEHOLDER: display of the eight scenarios.}
\label{fig:scenario_display}
\vspace{-15pt}
\end{figure}

\subsubsection{Creating a Challenging and Informative Benchmark}
A core challenge in designing any computer vision benchmark is limiting the ways the task can be solved \textit{other} than through the ability of interest -- in this case, visual understanding of physical scenes.
This has especially become an issue with testing deep learning-based models, which excel at learning ``shortcut solutions'' -- discriminating features that (usually unintentionally) correlate with the task solution, but have no causal relationship to it and therefore do not represent a generally useful computation outside of the benchmark dataset.
Along with creating our task in simulated scenarios without semantic and categorical information we try to prevent ``benchmark solving without physical understanding'' in three ways:

\paragraph{Physically irrelevant visual variation.}
First, we include substantial visual variation across task trials that is \textit{not relevant to the physical dynamics and outcome of the scene}: 
variation in camera position and pose, object colors and textures, the choice of ``distractor'' object models that do not participate in task-relevant dynamics, and the appearance and geometry of the background.
The across-trial variation that \textit{is} relevant for predicting physical outcomes -- objects' number, positions, poses, sizes, shapes, spatial and contact relationships, and initial velocities -- therefore cannot be gleaned easily from causally unrelated features.

\paragraph{Testing on multiple scenarios}
Second, we develop multiple scenarios that incorporate distinct (but overlapping) sets of physical phenomena.
Although there are many visual physics and reinforcement learning benchmarks that comprise several scenarios, these primarily probe the same few physical concepts (e.g., multi-object collisions or the effects of gravity) under different \textit{visual} conditions;
moreover, it is not common practice to train and test the same machine learning model across multiple scenarios: scores are usually reported for multiple models, each trained and tested on a single scenario.
In our view, this drastically limits the conclusions that can be drawn about whether a given model captures \textit{any} aspect of intuitive physical judgment.
If an algorithm is able to match human performance on a single scenario, it could be because the model uses the same physical concepts that humans would use to do that task -- but it also could be because the model has learned a representation or computation that is only valid for that scenario.
Given the possibility of shortcut learning and the relative ease of fitting to a narrower dataset over a broader one, the latter explanation is more likely.
In analogy to visual categorization benchmarks, a model that excels on a single scenario should be thought of like a model that detects objects or scenes from a single category: 
perhaps useful in specialized cases, but not a successful model of human-level understanding.
For this reason, we consider it most informative to benchmark individual trained models (not merely model architectures) across the full set of physical scenarios; we provide code to make this type of multi-scenario testing straightforward (as well as more standard, but less informative, within-scenario training and testing.) 

\paragraph{Comparing against both human accuracy and human error patterns}
Finally, we have collected (and encourage comparison against) the task responses of a large number of participants on a large number of distinct trials for which human performance is not perfect -- and in some cases is at or below chance.
By design, some stimuli in our benchmark are more challenging than others to physically reason about based on available visual information.
This implies that any super-human performance on these trials would mostly come from learning to solve the task \textit{via} non-physical factors (i.e., shortcuts.) 
Comparison between model and human or non-human primate \textit{error patterns} has been shown to allow much finer separation between better and worse models of animal vision than merely comparing overall task performance.
Thus, making the same accurate predictions \textit{and errors} is a strictly stronger test of whether a given model has learned human-like physical understanding than merely matching or exceeding performance on a particular test set. 
% If a single model were to make fewer errors than humans on many testing scenarios, this could be taken as evidence of true super-human physical understanding;
% otherwise, ``scenario overfitting'' via non-physical learning would be a more sensible interpretation of single scenario super-human performance with a non-human error pattern.


==> Sections/relatedwork.tex <==
\subsection{Related Work \textcolor{MyPurple}{Damian's draft}}

Prior work on benchmarking intuitive physics models varies greatly in its definition and evaluation of physical understanding. Physical simulation approaches define physical understanding as being able to accurately predict the motion of one or multiple objects. These benchmarks range from simple 2D datasets in which object positions have to be predicted at fixed time intervals to more realistic 3D benchmarks which focus on the step-by-step motion prediction of objects of different shapes which interact with one another. While the visual and geometric simplicity of 2D setups allows for longer term predictions \citep{bakhtin2019phyre}, most 3D benchmarks focus on a narrow subset of short term predictions such as whether a tower will fall \citep{groth2018shapestacks} or how objects will move behind an occluder \citep{riochet2018intphys, smith2019modeling}. \citet{bakhtin2019phyre} evaluate models on long-range 2D prediction scenarios in which a balls motion has to be predicted to judge whether it will end up in a specific target zone. \citet{groth2018shapestacks} propose a stability-based 3D task in which dynamics models need to predict whether a tower made up of objects of complex different shapes will fall or not. Others evaluate physical understanding as being able to distinguish real physical motion from counterfactuals that break physical laws \citep{riochet2018intphys, piloto2018probing, smith2019modeling}. All of these benchmarks focus and overfit on one or a few types of physical phenomena rather than learning a general understanding of physics, while our proposed benchmark can be seen as a superset of these scenarios. However, as we focus on constructing realistic 3D physical prediction problems, we choose to work with prediction horizons similar to prior 3D physics benchmarks \citep{riochet2018intphys, piloto2018probing, groth2018shapestacks} which are shorter than the 2D prediction problems presented in \citet{bakhtin2019phyre}.

Most datasets for learning and evaluating physical understanding however have not been introduced in their own right but rather as a side-effect of proposing new physics prediction models. As such, not all data is publicly released, making it impossible to evaluate other approaches on the exact same scenarios. 
Prior work has proposed many different approaches to physics prediction, which range from physics models that directly make predictions on 2D image pixels, \citep{fragkiadaki2015learning, agrawal2016learning, li2016fall, finn2016unsupervised, lerer2016learning, zhang2016comparative, mottaghi2016newtonian, mottaghi2016happens, vondrick2016anticipating, haber2018learning, lee2018stochastic, schmeckpeper2019learning, girdhar2020forward}, voxels or point clouds \citep{tran2015learning, tran2016deep, qi2017pointnet, qi2017pointnet++, byravan2017se3}, to physics predictors that operate on intermediate object-centric, graph-based representations that are assumed to be available or have been extracted from images \citep{chang2016compositional, battaglia2016interaction, li2018learning, bates2018modeling, tacchetti2018relational, sanchez2018graph, battaglia2018relational, mrowca2018flexible, ajay2019combining, smith2019modeling, ye2019compositional, kipf2019contrastive, villegas2019high, qi2020learning, veerapaneni2020entity, girdhar2020forward}.
While physics models that make predictions in image pixel space usually do not require object annotations as supervision, supervised object-centric physics predictors have been shown to make more accurate predictions for a wide variety of complex physical interactions between objects of different shapes and materials. Several works recently proposed methods to extract object-centric representations from images without supervision \citep{burgess2019monet, greff2019multi, bear2020learning}. These approaches have not yet been used to make physical dynamics predictions, but can be easily extended with object-centric dynamics prediction modules.
In this work, we aim to comprehensively cover the state-of-the-art of intuitive physics modeling by comparing a large set of physics prediction models with varying degrees of supervision and object priors built in against each other.
All models are compared to collected human responses on the exact same test stimuli.


% P1: Problems with collecting many aspects of intuitive physics into a single dataset/benchmark: What unifies them? How to get around language-level tasks for abilities that we think are pre-/non-linguistic?
Many high-quality benchmarks have helped push the development of visual algorithms for \textit{semantic} scene understanding -- how a person might describe the types of object present, the actions occurring, and the high-level content or relationships between things.
We mean to test an orthogonal set of human visual abilities -- ``visual intuitive physics'' (VIP) -- that do not require categorical classification or semantic understanding: those that allow us to perceive novel objects and predict how they will physically behave and interact with other objects, even without knowing what categories they belong to.
Although videos from existing vision datasets and benchmarks \textit{involve} physical phenomena, their use of everyday objects and scenes confounds tests of physical understanding with tests of semantic knowledge.
A model for predicting where cups stand in relation to plates and tables might learn only spatial correlations between these object categories, without ever learning what would happen if a cup were placed on its side or on the edge of a table.
This implies that a VIP benchmark task should not be solvable through semantic understanding of scenes or knowledge of which object configurations are common in the real world; 
rather, it should require judgments about objects' physical properties, relationships, and dynamics.

%Datasets: ShapeStacks \citep{groth2018shapestacks}, IntPhys \citep{riochet2018intphys}, PHYRE \cite{bakhtin2019phyre} 

%Towers fall \citep{lerer2016learning} A comparative evaluation of approximate probabilistic simulation and deep neural networks as accounts of human physical scene understanding \citep{zhang2016comparative},

%Probing physics knowledge using tools from developmental psychology \citep{piloto2018probing}, \citep{smith2019modeling}

%CVP \citep{ye2019compositional}, RPIN \citep{qi2020learning}, SVG \citep{lee2018stochastic}, C-SWM \citep{kipf2019contrastive}, OP3 \citep{veerapaneni2020entity}, RELATE \citep{ehrhardt2020relate}, Forward prediction for physical reasoning \citep{girdhar2020forward}, Learning predictive models from observation and interaction \citep{schmeckpeper2019learning}, High fidelity video prediction with large stochastic recurrent neural networks \citep{villegas2019high}, Anticipating visual representations from unlabeled video \citep{vondrick2016anticipating},
